Socratis: Are large multimodal models emotionally aware?

Existing emotion prediction benchmarks contain coarse emotion labels which do not consider the diversity of emotions that an image and text can elicit in humans due to various reasons. Learning diverse reactions to multimodal content is important as intelligent machines take a central role in generating and delivering content to society. To address this gap, we propose Socratis, a societal reactions benchmark, where each image-caption (IC) pair is annotated with multiple emotions and the reasons for feeling them. Socratis contains 18K free-form reactions for 980 emotions on 2075 image-caption pairs from 5 widely-read news and image-caption (IC) datasets. We benchmark the capability of state-of-the-art multimodal large language models to generate the reasons for feeling an emotion given an IC pair. Based on a preliminary human study, we observe that humans prefer human-written reasons over 2 times more often than machine-generated ones. This shows our task is harder than standard generation tasks because it starkly contrasts recent findings where humans cannot tell apart machine vs human-written news articles, for instance. We further see that current captioning metrics based on large vision-language models also fail to correlate with human preferences. We hope that these findings and our benchmark will inspire further research on training emotionally aware models.

==> sections/intro.tex <==
\section{Rewritten Introduction}
\color{blue}
A crucial prerequisite for effective communication and collaboration is the ability to possess emotional awareness \cite{goleman1996emotional}. Adapting one's communication style and tone can often facilitate more engaging interactions. Similarly, as intelligent machines become increasingly prevalent in our lives ranging from generative content creation to collaborative and embodied AI, it is important for them to possess similar emotional intelligence to foster a greater degree of trust and acceptance for their users. To address this research 
problem, existing emotion prediction works generally categorize reactions by coarse labels. However, this oversimplification ignores the possibility where the same content can elicit different emotional reactions due to various reasons. For instance, the image and caption in Figure~\ref{fig:teaserfig} can generate two possible conflicting emotions with valid reasons. Learning to understand these nuances is crucial for an AI to be able to tailor its interactions to individual emotional states.

To encourage further research on emotionally aware AI, we introduce the SOCRATIS benchmark - a dataset of detailed diverse reactions written by humans on images and captions. SOCRATIS includes 980 shades of emotions and 20K free-form reactions written by humans on 2075 image and caption pairs collected from 5 existing news and image-caption datasets. Given an image, a news caption and an emotion word, our task is to generate a caption that explains why the image and caption may elicit the specified emotion in a person. Unlike related benchmarks that formulate emotion prediction as a multiclass classification problem \cite{panda2018contemplating, yang2023emoset, dalmia2016columbia} or predicting reactions to artistic images \cite{mohamed2022artelingo, achlioptas2021artemis}, niche topics such as gun violence \cite{reardon-etal-2022-bu}, and morality \cite{jiang2021can}, SOCRATIS contains diverse reactions for various emotions on images and captions sourced from widely used news and image-caption datasets. Our task also bears strong similarity to the NICE Dataset \cite{chen2021nice} and MisInfoReaction Frames \cite{gabriel2021misinfo}, where their goals are to predict emotionally charged captions for images or the actions one is inclined to take after reading a text caption, respectively.

As an initial benchmark, we evaluate state-of-the-art unimodal and multimodal large language models on our SOCRATIS dataset to analyze the importance of using the visual context of the images to generate more accurate explanations. Additionally, we conduct a human study to evaluate the quality of the machine-generated explanations as well as assess the correlation between human judgment and common metrics including BART and CLIP scores.

Our results show a significant gap in current AI capabilities for this task. Humans prefer human-written responses twice as often as machine-generated ones. This starkly contrasts recent findings where humans could barely tell the difference between machine-generated and AI-generated news text \cite{zellers2019defending}. Furthermore, when we separate the generations into two groups - good generations as rated by humans (when humans can't discriminate between human-written and machine-generated) and poor generations (when humans pick human-written over machine-generated), we observe a negligible difference in how current metrics score the generated text. This highlights the failure of current generation metrics to distinguish the subtle differences between good and poor emotional reactions. We hope these initial results will spark further research and discussion on improving the emotional awareness of foundation models.
\color{black} 

\if
Sample abstract: Given the increasingly central role that AI is taking in our everyday lives ranging from content generation to interactive search engines, the importance of training emotionally aware AI cannot be understated. Existing emotion prediction benchmarks often contain coarse emotion labels for image and text pairs which does not consider the myriad of emotions that an image and text can elicit in humans due to various reasons. To address this limitation, we propose the Socratis benchmark - a dataset of multiple diverse emotions and reasons for feeling the emotion for each image-caption pair. Socratis contains 18K free-form reactions for 980 emotions on 2075 image-caption pairs from 5 widely-read news and image-caption datasets. We benchmark the capability of a state-of-the-art multimodal large language model to generate explanations. Based on a preliminary human study, we observe that current captioning metrics fail to not only correlate with human preferences but also capture the nuances between different emotions and social factors. We hope that Socratis will inspire further research on training emotionally aware AI.
\fi
